A Machine Learning-Based Approach For Detecting Malicious PyPI Packages

Background. In modern software development, the use of external libraries and packages is increasingly prevalent, streamlining the software development process and enabling developers to deploy feature-rich systems with little coding. While this reliance on reusing code offers substantial benefits, it also introduces serious risks for deployed software in the form of malicious packages - harmful and vulnerable code disguised as useful libraries. Aims. Popular ecosystems, such PyPI, receive thousands of new package contributions every week, and distinguishing safe contributions from harmful ones presents a significant challenge. There is a dire need for reliable methods to detect and address the presence of malicious packages in these environments. Method. To address these challenges, we propose a data-driven approach that uses machine learning and static analysis to examine the package's metadata, code, files, and textual characteristics to identify malicious packages. Results. In evaluations conducted within the PyPI ecosystem, we achieved an F1-measure of 0.94 for identifying malicious packages using a stacking ensemble classifier. Conclusions. This tool can be seamlessly integrated into package vetting pipelines and has the capability to flag entire packages, not just malicious function calls. This enhancement strengthens security measures and reduces the manual workload for developers and registry maintainers, thereby contributing to the overall integrity of the ecosystem.

==> equations/eq_similarity.tex <==
\begin{equation}
   Similarity ( \pmb{ST}_{A}, \pmb {ST}_{B})= 
    \tikzmarknode{similarity}{\highlight{gray}{cos(\pmb \theta) = \frac {\pmb{ST}_{A} \cdot \pmb{ST}_{B}}{||\pmb{ST}_{A}|| \cdot ||\pmb{ST}_{B}||}}}
\end{equation}

==> equations/eq_verification.tex <==
\vspace{1.1\baselineskip}

\begin{align*}\label{eq_ver}
likelyhood~of~Being~Unsafe  =
        % count_file
    \tikzmarknode{count_file}{\highlight{red}{(FC_{A} (\pm2)==FC_{B})}} \land 
    \\
    \tikzmarknode{Similarity of file names}
    {\highlight{gray}{SFN (ST(A),ST(B))> 0.98}} \land 
    \\
   \tikzmarknode{levenshtine}{\highlight{dkgreen}{LD(name(A),name(B)) [2,16]}} \\
   \tikzmarknode{packA}{\highlight{}{where~\pmb{A}~is~a~missclassified~package}} \\
     \tikzmarknode{packB}{\highlight{}{and~\pmb{B}~is~a~popular~ package}} 
\end{align*} 


% % Annotated part using Tikz
% \begin{tikzpicture}[overlay,remember picture,>=stealth,nodes={align=left,inner ysep=1pt},<-]
% %     % For "Dir" 
%     \path (count_file.north) ++ (7,1em) node[anchor=south east,color=red!67] (filescountlabel){files count};
%     \draw [color=red!87](dir.north) |- ([xshift=-0.3ex,color=red]dirlabel.south west);
    
%     % For "Own"
%     \path (own.south) ++ (0,-1em) node[anchor=north west,color=blue!67] (ownlabel){size of own code};
%     \draw [color=blue!57](own.south) |- ([xshift=-0.3ex,color=blue]ownlabel.south east);
    
%     % For "Trans" 
%     \path (tran.north) ++ (0,1em) node[anchor=south west,color=OliveGreen!67] (tranlabel){size of first level of transitive deps};
%     \draw [color=OliveGreen!87](tran.north) |- ([xshift=-0.3ex,color=green]tranlabel.south east);

% % For "Direct dependency (dir)" 
%     % \path (dir.north) ++ (0,1em) node[anchor=south west ,color=red!67] (dirlabel){Technical\\leverage};
%     % \draw [color=red!87](dir.north) |- ([xshift=-0.3ex,color=red]dirlabel.south east);
    
% \end{tikzpicture}
% \vspace{1.1\baselineskip}
%  \end{wrapfigure}


==> implications.tex <==
\section{Implication}\label{implications}
In this section, we highlight the most important implications of the results of our empirical study for both registry maintainers and researchers.\\
\noindent
\textbf{For registry maintainer.} To alleviate the cost and burden of  manual code reviewing for pre-selection packages by any proposed approach, previously reviewed packages should be reported, then a similarity check to those packages could be easily conducted. \\
Most proposed approaches are working impartially, thus to speed up the vetting process of the entire ecosystem, there is still a need for collaborative analysis from different tools result to overcome the repeated analysis as a result of indirect dependencies. As this kind of repetition results in wasting time and resources.\\
It is necessary to include the degree of suspicion per each vetted package per
day, to raise the awareness of developer reuse those packages, thus, help developers to make decisions about continuity of using those packages or not.\\
\noindent
\textbf{For researcher}. There is still a need to evaluate our approach on the entire PyPI ecosystem, to show its effectiveness and usability on a large scale. Moreover, we invite the researcher to advance the state-of-the-art in static analysis techniques to help for maintaining the integrity of PyPI ecosystem.




==> tables/RQ2_features.tex <==
\begin{tabular}{ll }

\toprule

\textbf{Feature}  & \textbf{Difference (\%)} \\ 

\midrule


 Has a license & 5.7 \\
    % \hline
 Has valid homepage  & 0.5\\
  % \hline

Has minimum configuration & -0.5\\

  % \hline
Has suspicious URL& -4.6  \\

 % \hline
 Has long string & -8.3 \\

 % \hline
 request (api) & -0.5  \\

 \bottomrule

 \end{tabular}




% \begin{tabular}{lll}

% \toprule

% \textbf{Feature} & \textbf{Package Type} & \textbf{Percentage (\%)}\\ 

% \midrule
% Has suspicious URL& malicious & 28  \\
%  & benign  & 9\\
 
%  \hline
%  Has mismatch license & malicious & 77 \\
%  & benign  & 1 \\
 
%   \hline
%  getattr (api) & malicious & 8 \\
%  & benign  & 54\\

  
%   \hline
% Has invalid or no author email& malicious & 54\\
%  & benign  &13 \\

  
%    \hline
%  Has invalid or no homepage & malicious & 80\\
%  & benign  & 27 \\


%   \hline

% Has minimum setup configuration & malicious & 79\\
%  & benign  &45\\


%  \hline
%  connect (api) & malicious & 15 \\
%  & benign  & 7\\

%  \hline
%  Has long string & malicious &7 \\
%  & benign  &0\\

% \hline
%  subprocess (api) & malicious & 12 \\
%  & benign  &24\\

%  \hline
%  request (api) & malicious & 66  \\
%  & benign  & 21\\
%  \bottomrule

%  \end{tabular}

%  \textbf{Q25\%} &  \textbf{Median}& \textbf{Q75\%} 

 

==> tables/comparison.tex <==
\begin{tabular}{ll|ll|ll|l}
\toprule
 Package & Type & \# Packj Alerts&  & \# Bandit Alerts & & Our Approach\\

         &      &  setup.py &   whole package & setup.py & whole package& \\

         
\midrule
 urllib3-1.26.11 & & 3 & 142 & 0 & 1257 & benign \\
 requests-2.28.1&\rotatebox{8}{benign} & 8 & 61 & 5 & 539 & benign \\
 % setuptools-64.0.3& &1 & 839& 0 & 1696 & benign \\
Acquisition-4.10& &3 & 29& 0 & 8 & benign \\
\bottomrule
 urlib3-1.21.1 & & 0 & 95& 0 & 56 & malicious \\
  request-1.0.117 &\rotatebox{7}{malicious} & 8 & 19 & 3 & 11 & malicious \\
   Acqusition-4.4.2 & &0 & 33 & 0 & 9 & malicious \\


 
\end{tabular}

==> tables/diff.tex <==
\begin{tabular}{lrrrrrrr}

\toprule

& \textbf{Mean}& \textbf{Min} & \textbf{Q25\%} &  \textbf{Median}& \textbf{Q75\%} & \textbf{Max}\\ 
\midrule
 \textbf{different (days)}  &
 308&
 2&
 55&
 114&
 395&
 1453 \\
 
 
 \bottomrule
 \end{tabular}

==> tables/final_dataset.tex <==
\begin{tabular}{ll}
\toprule
\textbf{Dataset} &\textbf{ Total} \\
\hline
popular & 5,193 \\
malicious & 138  \\
\hline

 \bottomrule
\end{tabular}

==> tables/new_july_malicious.tex <==
\begin{tabular}{ll|ll|ll}
\toprule
 Malicious Package &  & \# Packj Alerts&  & \# Bandit Alerts & \\
         &      &     whole pkg& setup & whole pkg& setup & 
\bottomrule

trexcolors-0.0.0	&&3	&0& 2& 0 \\
brokescolors-0.0.0	&&3&0 & 2& 0\\
 brokesrcl-0.0.0		&&0& 0& 1 &0 \\
 brokescolors2-0.0.0 &&0	&0 &1 &0\\
brokescolors3-0.0.0	&&3&0 &2 & 0 \\
 \hline
\end{tabular}

%\footnotesize
% \begin{flushleft}

% \threeStars \space In contrast to other tools, our approach accurately identifies malicious packages.  \\
% \end{flushleft}



==> tables/ohm_approach.tex <==
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{lll|c}
      
     \toprule
 \end{tabular}
 \end{adjustbox}


==> tables/performance_practice_classifier.tex <==
\begin{tabular}{llllll}
\toprule
\textbf{Dataset} &\textbf{Package type} &\textbf{ Total} & \textbf{#FP} &\textbf{FN} \\

\hline
Train&popular & 5,193 & 3  &- \\
&malicious & 138  & -  & 26  \\
\hline
External&typical & 397 & 0 &-  \\
& malicious & 143  &- &38  &  
 \midrule    
 \bottomrule
\end{tabular}

==> tables/performance_test_dataset.tex <==
\begin{tabular}{lllll}
\toprule
 & &  \textbf{Overall}& & \\

   & \textbf{Precission (\%)} & \textbf{Recall (\%)} & \textbf{F1-score (\%)} & 
\\
\midrule
\textbf{Train}&98&91&94\\
\textbf{External} &91&100&95\\

\end{tabular}



==> tables/similiraty_typo.tex <==
\begin{tabular}{l|l}
   \textbf{Popular pkgs} &  \textbf{Subset of 31 malicious packages} \\
   \toprule
     & 2022-requests-3.0.0, advenced-requests-3.0.0 ,\\
  requests-2.28.1                    & android-plus-new-5.3.1, apple-tv-new-1.0.0,\\ & BeautifulSoup-new-3.0.0, \\
               & chillie-1.0.0, dont-test-me-1.1.1,\\
                     % & free-requests-module-3.0.0, http-interact-3.0.0,\\
                     % & new-reque-20222-2.28.1, new-request-2022-4.5.1,\\
                     % & oklend-0.9.1, youtube-new-2.2.1 ....\\
    \midrule
\end{tabular}

==> tables/statistics_external_comparison_tool.tex <==
\begin{tabular}{c|c}
     &  \\
     & 
\end{tabular}



packj_alerts_count_whole	packj_alerts_count_setup	alerts_count_whole	alerts_count_setup
count	50.000000	50.000000	50.000000	50.000000
mean	39.260000	1.980000	86.840000	0.420000
std	74.976407	3.846493	233.663141	1.162158
min	0.000000	0.000000	0.000000	0.000000
25%	3.500000	0.000000	3.000000	0.000000
50%	11.500000	1.000000	14.500000	0.000000
75%	40.750000	2.000000	59.000000	0.000000
max	417.000000	21.000000	1548.000000	7.000000
1
​
